Rethinking Reconstruction-based Graph-Level Anomaly Detection: Limitations and a Simple Remedy

Graph autoencoders (Graph-AEs) learn representations of given graphs by aiming to accurately reconstruct them. A notable application of Graph-AEs is graph-level anomaly detection (GLAD), whose objective is to identify graphs with anomalous topological structures and/or node features compared to the majority of the graph population. Graph-AEs for GLAD regard a graph with a high mean reconstruction error (i.e. mean of errors from all node pairs and/or nodes) as anomalies. Namely, the methods rest on the assumption that they would better reconstruct graphs with similar characteristics to the majority. We, however, report non-trivial counter-examples, a phenomenon we call reconstruction flip, and highlight the limitations of the existing Graph-AE-based GLAD methods. Specifically, we empirically and theoretically investigate when this assumption holds and when it fails. Through our analyses, we further argue that, while the reconstruction errors for a given graph are effective features for GLAD, leveraging the multifaceted summaries of the reconstruction errors, beyond just mean, can further strengthen the features. Thus, we propose a novel and simple GLAD method, named MUSE. The key innovation of MUSE involves taking multifaceted summaries of reconstruction errors as graph features for GLAD. This surprisingly simple method obtains SOTA performance in GLAD, performing best overall among 14 methods across 10 datasets.

==> format_instructions.tex <==

\section{Submission of papers to NeurIPS 2024}


Please read the instructions below carefully and follow them faithfully.


\subsection{Style}


Papers to be submitted to NeurIPS 2024 must be prepared according to the
instructions presented here. Papers may only be up to {\bf nine} pages long,
including figures. Additional pages \emph{containing only acknowledgments and
references} are allowed. Papers that exceed the page limit will not be
reviewed, or in any other way considered for presentation at the conference.


The margins in 2024 are the same as those in previous years.


Authors are required to use the NeurIPS \LaTeX{} style files obtainable at the
NeurIPS website as indicated below. Please make sure you use the current files
and not previous versions. Tweaking the style files may be grounds for
rejection.


\subsection{Retrieval of style files}


The style files for NeurIPS and other conference information are available on
the website at
\begin{center}
  \url{http://www.neurips.cc/}
\end{center}
The file \verb+neurips_2024.pdf+ contains these instructions and illustrates the
various formatting requirements your NeurIPS paper must satisfy.


The only supported style file for NeurIPS 2024 is \verb+neurips_2024.sty+,
rewritten for \LaTeXe{}.  \textbf{Previous style files for \LaTeX{} 2.09,
  Microsoft Word, and RTF are no longer supported!}


The \LaTeX{} style file contains three optional arguments: \verb+final+, which
creates a camera-ready copy, \verb+preprint+, which creates a preprint for
submission to, e.g., arXiv, and \verb+nonatbib+, which will not load the
\verb+natbib+ package for you in case of package clash.


\paragraph{Preprint option}
If you wish to post a preprint of your work online, e.g., on arXiv, using the
NeurIPS style, please use the \verb+preprint+ option. This will create a
nonanonymized version of your work with the text ``Preprint. Work in progress.''
in the footer. This version may be distributed as you see fit, as long as you do not say which conference it was submitted to. Please \textbf{do
  not} use the \verb+final+ option, which should \textbf{only} be used for
papers accepted to NeurIPS.


At submission time, please omit the \verb+final+ and \verb+preprint+
options. This will anonymize your submission and add line numbers to aid
review. Please do \emph{not} refer to these line numbers in your paper as they
will be removed during generation of camera-ready copies.


The file \verb+neurips_2024.tex+ may be used as a ``shell'' for writing your
paper. All you have to do is replace the author, title, abstract, and text of
the paper with your own.


The formatting instructions contained in these style files are summarized in
Sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.


\section{General formatting instructions}
\label{gen_inst}


The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).  Use 10~point
type with a vertical spacing (leading) of 11~points.  Times New Roman is the
preferred typeface throughout, and will be selected for you by default.
Paragraphs are separated by \nicefrac{1}{2}~line space (5.5 points), with no
indentation.


The paper title should be 17~point, initial caps/lower case, bold, centered
between two horizontal rules. The top rule should be 4~points thick and the
bottom rule should be 1~point thick. Allow \nicefrac{1}{4}~inch space above and
below the title to rules. All pages should start at 1~inch (6~picas) from the
top of the page.


For the final version, authors' names are set in boldface, and each name is
centered above the corresponding address. The lead author's name is to be listed
first (left-most), and the co-authors' names (if different address) are set to
follow. If there is only one co-author, list both author and co-author side by
side.


Please pay special attention to the instructions in Section \ref{others}
regarding figures, tables, acknowledgments, and references.


\section{Headings: first level}
\label{headings}


All headings should be lower case (except for first word and proper nouns),
flush left, and bold.


First-level headings should be in 12-point type.


\subsection{Headings: second level}


Second-level headings should be in 10-point type.


\subsubsection{Headings: third level}


Third-level headings should be in 10-point type.


\paragraph{Paragraphs}


There is also a \verb+\paragraph+ command available, which sets the heading in
bold, flush left, and inline with the text, with the heading followed by 1\,em
of space.


\section{Citations, figures, tables, references}
\label{others}


These instructions apply to everyone.


\subsection{Citations within the text}


The \verb+natbib+ package will be loaded for you by default.  Citations may be
author/year or numeric, as long as you maintain internal consistency.  As to the
format of the references themselves, any style is acceptable as long as it is
used consistently.


The documentation for \verb+natbib+ may be found at
\begin{center}
  \url{http://mirrors.ctan.org/macros/latex/contrib/natbib/natnotes.pdf}
\end{center}
Of note is the command \verb+\citet+, which produces citations appropriate for
use in inline text.  For example,
\begin{verbatim}
   \citet{hasselmo} investigated\dots
\end{verbatim}
produces
\begin{quote}
  Hasselmo, et al.\ (1995) investigated\dots
\end{quote}


If you wish to load the \verb+natbib+ package with options, you may add the
following before loading the \verb+neurips_2024+ package:
\begin{verbatim}
   \PassOptionsToPackage{options}{natbib}
\end{verbatim}


If \verb+natbib+ clashes with another package you load, you can add the optional
argument \verb+nonatbib+ when loading the style file:
\begin{verbatim}
   \usepackage[nonatbib]{neurips_2024}
\end{verbatim}


As submission is double blind, refer to your own published work in the third
person. That is, use ``In the previous work of Jones et al.\ [4],'' not ``In our
previous work [4].'' If you cite your other papers that are not widely available
(e.g., a journal paper under review), use anonymous author names in the
citation, e.g., an author of the form ``A.\ Anonymous'' and include a copy of the anonymized paper in the supplementary material.


\subsection{Footnotes}


Footnotes should be used sparingly.  If you do require a footnote, indicate
footnotes with a number\footnote{Sample of the first footnote.} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches (12~picas).


Note that footnotes are properly typeset \emph{after} punctuation
marks.\footnote{As in this example.}


\subsection{Figures}


\begin{figure}
  \centering
  \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Sample figure caption.}
\end{figure}


All artwork must be neat, clean, and legible. Lines should be dark enough for
purposes of reproduction. The figure number and caption always appear after the
figure. Place one line space before the figure caption and one line space after
the figure. The figure caption should be lower case (except for first word and
proper nouns); figures are numbered consecutively.


You may use color figures.  However, it is best for the figure captions and the
paper body to be legible if the paper is printed in either black/white or in
color.


\subsection{Tables}


All tables must be centered, neat, clean and legible.  The table number and
title always appear before the table.  See Table~\ref{sample-table}.


Place one line space before the table title, one line space after the
table title, and one line space after the table. The table title must
be lower case (except for first word and proper nouns); tables are
numbered consecutively.


Note that publication-quality tables \emph{do not contain vertical rules.} We
strongly suggest the use of the \verb+booktabs+ package, which allows for
typesetting high-quality, professional tables:
\begin{center}
  \url{https://www.ctan.org/pkg/booktabs}
\end{center}
This package was used to typeset Table~\ref{sample-table}.


\begin{table}
  \caption{Sample table title}
  \label{sample-table}
  \centering
  \begin{tabular}{lll}
    \toprule
    \multicolumn{2}{c}{Part}                   \\
    \cmidrule(r){1-2}
    Name     & Description     & Size ($\mu$m) \\
    \midrule
    Dendrite & Input terminal  & $\sim$100     \\
    Axon     & Output terminal & $\sim$10      \\
    Soma     & Cell body       & up to $10^6$  \\
    \bottomrule
  \end{tabular}
\end{table}

\subsection{Math}
Note that display math in bare TeX commands will not create correct line numbers for submission. Please use LaTeX (or AMSTeX) commands for unnumbered display math. (You really shouldn't be using \$\$ anyway; see \url{https://tex.stackexchange.com/questions/503/why-is-preferable-to} and \url{https://tex.stackexchange.com/questions/40492/what-are-the-differences-between-align-equation-and-displaymath} for more information.)

\subsection{Final instructions}

Do not change any aspects of the formatting parameters in the style files.  In
particular, do not modify the width or length of the rectangle the text should
fit into, and do not change font sizes (except perhaps in the
\textbf{References} section; see below). Please note that pages should be
numbered.


\section{Preparing PDF files}


Please prepare submission files with paper size ``US Letter,'' and not, for
example, ``A4.''


Fonts were the main cause of problems in the past years. Your PDF file must only
contain Type 1 or Embedded TrueType fonts. Here are a few instructions to
achieve this.


\begin{itemize}


\item You should directly generate PDF files using \verb+pdflatex+.


\item You can check which fonts a PDF files uses.  In Acrobat Reader, select the
  menu Files$>$Document Properties$>$Fonts and select Show All Fonts. You can
  also use the program \verb+pdffonts+ which comes with \verb+xpdf+ and is
  available out-of-the-box on most Linux machines.


\item \verb+xfig+ "patterned" shapes are implemented with bitmap fonts.  Use
  "solid" shapes instead.


\item The \verb+\bbold+ package almost always uses bitmap fonts.  You should use
  the equivalent AMS Fonts:
\begin{verbatim}
   \usepackage{amsfonts}
\end{verbatim}
followed by, e.g., \verb+\mathbb{R}+, \verb+\mathbb{N}+, or \verb+\mathbb{C}+
for $\mathbb{R}$, $\mathbb{N}$ or $\mathbb{C}$.  You can also use the following
workaround for reals, natural and complex:
\begin{verbatim}
   \newcommand{\RR}{I\!\!R} %real numbers
   \newcommand{\Nat}{I\!\!N} %natural numbers
   \newcommand{\CC}{I\!\!\!\!C} %complex numbers
\end{verbatim}
Note that \verb+amsfonts+ is automatically loaded by the \verb+amssymb+ package.


\end{itemize}


If your file contains type 3 fonts or non embedded TrueType fonts, we will ask
you to fix it.


\subsection{Margins in \LaTeX{}}


Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+ from the \verb+graphicx+ package. Always specify the
figure width as a multiple of the line width as in the example below:
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
See Section 4.4 in the graphics bundle documentation
(\url{http://mirrors.ctan.org/macros/latex/required/graphics/grfguide.pdf})


A number of width problems arise when \LaTeX{} cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command when
necessary.

\begin{ack}
Use unnumbered first level headings for the acknowledgments. All acknowledgments
go at the end of the paper before the list of references. Moreover, you are required to declare
funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work).
More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2024/PaperInformation/FundingDisclosure}.


Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to automatically hide this section in the anonymized submission.
\end{ack}

\section*{References}


References follow the acknowledgments in the camera-ready paper. Use unnumbered first-level heading for
the references. Any choice of citation style is acceptable as long as you are
consistent. It is permissible to reduce the font size to \verb+small+ (9 point)
when listing the references.
Note that the Reference section does not count towards the page limit.
\medskip


{
\small


[1] Alexander, J.A.\ \& Mozer, M.C.\ (1995) Template-based algorithms for
connectionist rule extraction. In G.\ Tesauro, D.S.\ Touretzky and T.K.\ Leen
(eds.), {\it Advances in Neural Information Processing Systems 7},
pp.\ 609--616. Cambridge, MA: MIT Press.


[2] Bower, J.M.\ \& Beeman, D.\ (1995) {\it The Book of GENESIS: Exploring
  Realistic Neural Models with the GEneral NEural SImulation System.}  New York:
TELOS/Springer--Verlag.


[3] Hasselmo, M.E., Schnell, E.\ \& Barkai, E.\ (1995) Dynamics of learning and
recall at excitatory recurrent synapses and cholinergic modulation in rat
hippocampal region CA3. {\it Journal of Neuroscience} {\bf 15}(7):5249-5262.
}

==> math_draft.tex <==
\section{Math draft}

Community structure.
Two groups, each has $N$ nodes.
Intra-community $p$.
Inter-community $1 - p$.

\subsection{$A$}
(1) If $i = j$,
\begin{equation*}
    \mathbb{E}[A_{ij}] = 0
\end{equation*}

(2) If $i$ and $j$ are in the same group,
\begin{equation*}
    \mathbb{E}[A_{ij}] = p
\end{equation*}

(3) If $i$ and $j$ are in different groups,
\begin{equation*}
    \mathbb{E}[A_{ij}] = 1 - p
\end{equation*}

\subsection{$A^2$}
(1) If $i = j$,
\begin{equation*}
    \mathbb{E}[A^2_{ij}] = (N - 1) p^2 + N (1-p)^2
\end{equation*}

(2) If $i$ and $j$ are in the same group,
\begin{equation*}
    \mathbb{E}[A^2_{ij}] = (N - 2) p^2 + N (1 - p)^2
\end{equation*}

(3) If $i$ and $j$ are in different groups,
\begin{equation*}
    \mathbb{E}[A^2_{ij}] = 2 (N - 1) p (1 - p)
\end{equation*}

\subsection{$A^3$}
(1) If $i = j$,
\begin{align*}
    \mathbb{E}[A^3_{ij}] 
    &= 
    (N - 1) (N - 2) p^3 +  % SS    
    2 N (N - 1) p (1 - p)^2 +  % SD/DS
    N (N - 1) p (1 - p)^2  % DD
    \\
    &= 
    (N - 1) (N - 2) p^3 + 
    3 N (N - 1) p (1 - p)^2    
\end{align*}

(2) If $i$ and $j$ are in the same group,
\begin{align*}
    \mathbb{E}[A^3_{ij}] 
    &= 
    (N - 2) (N - 3) p^3 +  % SS 
    p +  % SS, ji 
    2 N (N - 2) p (1 - p)^2 +  % SD/DS
    2 N p (1 - p) +  % SD, jx / DS, xi    
    N (N - 1) p (1 - p)^2  % DD
    \\
    &= (N - 2) (N - 3) p^3 + 
    N (3N - 5) p (1 - p)^2 +
    p + 2 N p (1 - p)
\end{align*}

(3) If $i$ and $j$ are in different groups,
\begin{align*}
    \mathbb{E}[A^3_{ij}] 
    &= 
    % say i in group 1, j in group 2
    2 (N - 1) (N - 2) p^2 (1 - p) +  % 11 / 22
    2 (N - 1) p (1 - p)  % 11, xi / 22, jx    
    \\&~~~~+
    (N - 1)^2 p^2 (1 - p) +  % 12
    (N - 1)^2 (1 - p)^3 + % 21
    (1 - p)  % 21, ji
    \\
    &= 
    (N - 1) (3N - 5) p^2 (1 - p) +
    (N - 1)^2 (1 - p)^3 +
    2 (N - 1) p (1 - p) + (1 - p)
\end{align*}

\newpage

\subsection{$A^4$}
(1) If $i = j$,
\begin{align*}
    \mathbb{E}[A^4_{ij}] 
    &= (N - 1) (N - 2) (N - 3) p^4 + % SSS
    (N - 1) (N - 2) p^2 + % SSS, first = last
    (N - 1) (N - 2) p^2 + % SSS, middle i
    (N - 1) p % SSS, first = last, middle i
    \\&~~~~+
    2 (N - 1) (N - 2) N p^2 (1 - p)^2 + % SSD / DSS    
    2 N (N - 1) p (1 - p)^2 + % SSD / DSS, middle i
    (N - 1) (N - 2) N p^2 (1 - p)^2 % SDS    
    (N - 1) N p (1 - p) % SDS, F=L
    \\&~~~~+
    2 N^2 (N - 1) p^2 (1 - p)^2 + % SDD / DDS    
    N (N - 1)^2 (1 - p)^4 + % DSD
    N (N - 1) (1 - p)^2 + % DSD, middle i
    N (N - 1) (1 - p)^2 % DSD, F = L
    N (1 - p) % DSD, F = L, middle i
    \\&~~~~+
    N (N - 1) (N - 2) p^2 (1 - p)^2 + % DDD
    N (N - 1) p (1 - p) % DDD, F = L
    \\
    % &= (N - 1) (N - 2) (N - 3) p^4 +
    % 2 N (3N^2 - 7N + 4) p^2 (1 - p)^2 +
    % N (N - 1)^2 (1 - p)^4
    % \\&~~~~+
    % % below: F = L
    % (N - 1) (N - 2) p^2 +
    % (N - 1) N p (1 - p) +
    % (N - 1) p 
    % \\&~~~~+
    % N (N - 1) (1 - p)^2 +         
    % N (N - 1) p (1 - p) +
    % % below: middle i
    % (N - 1) p +    
    % 2 N (N - 1) p (1 - p)^2
    % \\&~~~~+
    % N (N - 1) (1 - p)^2 + 
    % N (1 - p)
    % \\
    &=
    (-6 + 11 N - 6 N^2 + N^3) p^4 + 
    2 (-1 + N) p^2 (-2 + N - 4 N (1-p)^2 + 3 N^2 (1-p)^2)
    \\&~~~~+
    N (1-p) (1 + 2 (-1 + N) (1-p) + (-1 + N)^2 (1-p)^3) 
    \\&~~~~+
    p (-1 + 2 N^2 (1-p) (1 + (1-p)) + N (1 - 2 (1-p) - 2 (1-p)^2))
\end{align*}

(2) If $i$ and $j$ are in the same group,
\begin{align*}
    \mathbb{E}[A^4_{ij}] 
    &=
    (N - 2) (N - 3) (N - 4) p^4 + % SSS
    (N - 2) (N - 3) p^3 + % SSS, F = L
    2 (N - 2) (N - 3) p^3 + % SSS, middle i / j
    2 (N - 2) p^3 % SSS, i jix j / i xji j
    \\&~~~~+
    (N - 2) p^3 + % SSS, i jxi j
    2 (N - 2) (N - 3) p^4 + % SSS, i jxy j / i yxi j
    2 (N - 2) p^2 % SSS, F = L, middle i / j
    \\&~~~~+
    2 (N - 2) (N - 3) N p^2 (1 - p)^2 + % SSD / DSS
    2 (N - 2) N p (1 - p)^2 + % SSD (i SiD j) / DSS (i DjS j)
    2 N p (1 - p)^2 + % SSD (i jiD j) / DSS (i Dji j)
    2 (N - 2) N p^2 (1 - p)^2 % SSD (i jSD j) / DSS (i DSi j)        
    \\&~~~~+
    (N - 2) (N - 3) N p^2 (1 - p)^2 + % SDS
    2 (N - 2) N p^2 (1 - p)^2 + % SDS (i jDS j / i SDi j)
    N p (1 - p)^2 + % SDS (i jDi j)
    2 N (N - 1) (N - 2) p^2 (1 - p)^2 % SDD / DDS
    \\&~~~~+
    2 N (N - 1) p^2 (1 - p)^2 + % SDD (i jDD j) / DDS (i DDi j)
    N (N - 1) (N - 2) (1 - p)^4 + % DSD
    N (N - 2) (1 - p)^3 + % DSD, F = L
    2 N (N - 1) (1 - p)^4 % DSD (i DiD j / i DjD j)
    \\&~~~~+
    2 N (1 - p)^2 + % DSD, F = L, middle i/j
    N (N - 1) (N - 2) p^2 (1 - p)^2 + % DDD
    N (N - 1) p (1 - p)^2 % DDD, F = L
    \\
    &= 
    3 (-2 + N)^2 p^3 + 
    (-3 + N) (-2 + N)^2 p^4 + 
    N (-2 + 3 N) p (1-p)^2 
    \\&~~~~+
    N (1-p)^2 (2 + (-2 + N) (1-p) + (-1 + N) N (1-p)^2) 
    \\&~~~~+
    2 p^2 (-2 + N + 7 N (1-p)^2 - 9 N^2 (1-p)^2 + 3 N^3 (1-p)^2)
\end{align*}

(3) If $i$ and $j$ are in different groups,
\begin{align*}
    \mathbb{E}[A^4_{ij}] 
    &=
    % suppose i in group 1 and j in group 2
    (N - 1) (N - 2) (N - 3) p^3 (1 - p) + % 111
    (N - 1) (N - 2) p^3 (1 - p) + % 111, right i
    (N - 1) (N - 2) p^2 (1 - p) % 111, middle i    
    \\&~~~~+
    (N - 1) (N - 2) p^2 (1 - p) + % 111, F = L
    (N - 1) p (1 - p) + % 111, middle i, F = L
    %
    (N - 1)^2 (N - 2) p^3 (1 - p) % 112
    \\&~~~~+
    (N - 1) (N - 2) p^2 (1 - p) + % 112, middle i
    %
    (N - 1)^2 (N - 2) p (1 - p)^3 + % 121    
    (N - 1)^2 p (1 - p)^3 % 121, right i
    \\&~~~~+
    (N - 1) (N - 2) p (1 - p)^2 + % 121, middle j
    (N - 1) p (1 - p)^2 + % 121, right i, middle j, i xji j
    (N - 1)^2 p (1 - p)^2 + % 121, F = L
    (N - 1) p (1 - p) % 121, F = L, middle j
    \\&~~~~+
    %
    (N - 1)^2 (N - 2) p^3 (1 - p) + % 122
    (N - 1)^2 p^2 (1 - p) + % 122, middle j    
    %
    (N - 1)^2 (N - 2) p (1 - p)^3 % 211
    \\&~~~~+
    (N - 1)^2 p (1 - p)^2 + % 211, middle i
    (N - 1) (N - 2) p (1 - p)^3 + % 211, left j
    (N - 1)^2 p (1 - p)^3 + % 211, right i
    (N - 1) p (1 - p)^2 % 211, middle i, left j
    \\&~~~~+
    (N - 1) p (1 - p)^2 + % 211, right i, left j
    %
    (N - 1)^2 (N - 2) p (1 - p)^3 + % 212
    (N - 1) (N - 2) p (1 - p)^2 % 212, middle i
    \\&~~~~+
    (N - 1)^2 p (1 - p)^3 + % 212, left j
    (N - 1)^2 p (1 - p)^2 + % 212, F = L
    (N - 1) p (1 - p)^2 + % 212, middle i, left j
    (N - 1) p (1 - p) % 212, middle i, F = L
    \\&~~~~+
    %
    (N - 1)^2 (N - 2) p (1 - p)^3 + % 221
    (N - 1)^2 p (1 - p)^3 + % 221, middle j
    (N - 1)^2 p (1 - p)^3 + % 221, left j
    (N - 1) (N - 2) p (1 - p)^3 % 221, right i
    \\&~~~~+
    (N - 1) p (1 - p)^2 + % 221, middle j, right i
    (N - 1) p (1 - p)^2 + % 221, left j, right i
    %    
    (N - 1) (N - 2) (N - 3) p^3 (1 - p) % 222
    \\&~~~~+
    (N - 1) (N - 2) p^2 (1 - p) + % 222, middle j
    (N - 1) (N - 2) p^2 (1 - p) + % 222, F = L
    (N - 1) p (1 - p) % 222, middle j, F = L
    \\
    &= (-1 + N) p (1-p) \triangle,
\end{align*}
where
\[
\triangle = 4 + (-11 + 6 N) p + (14 - 15 N + 4 N^2) p^2 + (-1 + 
      5 N) (1-p) + (-1 - 5 N + 4 N^2) (1-p)^2
\]

\newpage

\subsection{$A^2 - A$}

(1) If $i = j$,
\begin{equation*}
    \mathbb{E}[A^2_{ij} - A_{ij}] 
    = (N - 1) p^2 + N (1 - p)^2,
\end{equation*}
which is positive for all $N > 1$ and $p > 0$.

(2) If $i$ and $j$ are in the same group,
\begin{align*}
    \mathbb{E}[A^2_{ij} - A_{ij}] 
    &= (N - 2) p^2 + N (1 - p)^2 - p \\
    &= p ((N - 2) p - 1) + N (1 - p)^2,
\end{align*}
which is positive for all $N \geq 4$ and $p > 0.5$.

(3) If $i$ and $j$ are in different groups,
\begin{align*}
    \mathbb{E}[A^2_{ij} - A_{ij}] 
    &= 2 (N - 1) p (1 - p) - (1 - p) \\
    &= (1 - p) (2 (N - 1) p - 1),
\end{align*}
which is positive for all $N \geq 2$ and $p > 0.5$.

\newpage

\subsection{$A^4 - A^3$}
(1) If $i = j$,
\begin{align*}
    \mathbb{E}[A^4_{ij} - A^3_{ij}] 
    &= 
    N^2 p (5 - 22 p + 34 p^2 - 22 p^3) - 
    p (1 - 4 p + 2 p^2 + 6 p^3) 
    \\&~~~~+
    N p (-1 + 6 p - 16 p^2 + 20 p^3) + 
    N^3 (1 - 4 p + 12 p^2 - 16 p^3 + 8 p^4).
\end{align*}
When $0.5 < p \leq 1$, we have
\begin{align*}
    p (5 - 22 p + 34 p^2 - 22 p^3) &> -0.125 \\
    -p (1 - 4 p + 2 p^2 + 6 p^3) &\geq -5 \\
    p (-1 + 6 p - 16 p^2 + 20 p^3) &> 0.25 \\
    1 - 4 p + 12 p^2 - 16 p^3 + 8 p^4 &> 0.5
\end{align*}
Hence, for all $N \geq 3$,
\[
\mathbb{E}[A^4_{ij} - A^3_{ij}]
> -0.125 N^2 - 5 + 0.25N + 0.5N^3
> 0
\]

(2) If $i$ and $j$ are in the same group,
\begin{align*}
    \mathbb{E}[A^4_{ij} - A^3_{ij}] 
    &= 
    -p (1 + 4 p - 6 p^2 + 12 p^3) + 
    N p (3 + 8 p - 30 p^2 + 30 p^3) 
    \\&~~~~+
    N^2 (p - 21 p^2 + 41 p^3 - 26 p^4) + 
    N^3 (1 - 4 p + 12 p^2 - 16 p^3 + 8 p^4)
\end{align*}
When $0.5 < p \leq 1$, we have
\begin{align*}
    -p (1 + 4 p - 6 p^2 + 12 p^3) &\geq -11 \\
    p (3 + 8 p - 30 p^2 + 30 p^3) &> -1.5 \\
    p - 21 p^2 + 41 p^3 - 26 p^4 &> -5 \\
    1 - 4 p + 12 p^2 - 16 p^3 + 8 p^4 &> 0.5
\end{align*}
Hence, for all $N \geq 11$,
\[
\mathbb{E}[A^4_{ij} - A^3_{ij}] 
> -11 - 1.5N -5N^2 + 0.5N^3 
> 0.
\]

(3) If $i$ and $j$ are in different groups,
\begin{align*}
    \mathbb{E}[A^4_{ij} - A^3_{ij}] 
    &= (1 - p) 
    (-2 + 2 p + 2 p^2 - 13 p^3 + 
    4 N^3 p (1 - 2 p + 2 p^2) 
    \\&~~~~-
    N^2 (1 + 2 p - 15 p^2 + 28 p^3) + 
    N (2 - 4 p - 9 p^2 + 33 p^3))
\end{align*}
When $0.5 < p \leq 1$, we have
\begin{align*}
    -2 + 2 p + 2 p^2 - 13 p^3 &\geq -11 \\
    4p (1 - 2 p + 2 p^2) &> 1 \\
    -(1 + 2 p - 15 p^2 + 28 p^3) &> -16 \\
    1 - 4 p + 12 p^2 - 16 p^3 + 8 p^4 &> 0.5
\end{align*}
Hence, for all $N \geq 17$,
\[
\mathbb{E}[A^4_{ij} - A^3_{ij}] = (1 - p) (-11 + N^3 -16 N^2 + 0.5N) \geq 0,
\]
and is strictly positive when $p \neq 1$.

\newpage

\subsection{Gradient}
Note that the expected gradient of the reconstruction error with respect to the parameter $W$, which is initialized as $\mathbf{I}$, is defined as $\mathbb{E}_{A}[\mathbf{A}^{4} - \mathbf{A}^{3}]$.
We study several properties of this gradient and the updated parameter $W'$.

First, as shown in the above proof, $\mathbb{E}_{A}[\mathbf{A}^{4} - \mathbf{A}^{3}]$ consist of three kinds of elements: (1) $i$ and $j$ are equal, (2) $v_{i}$ and $v_{j}$ belong to the same group, and (3) $v_{i}$ and $v_{j}$ belong to the different groups.
Thus, we can express $\mathbb{E}_{A}[\mathbf{A}^{4} - \mathbf{A}^{3}]$ as $a\mathbf{I} + b\mathbf{P} + c\mathbf{U}$, where $a,b,c \in \mathbb{R}$ and $\mathbf{P}$ and $\mathbf{U}$ are defined as:
\begin{equation}
    \mathbf{P} = \begin{pmatrix}
    \mathbf{1} & \mathbf{0} \\
    \mathbf{0} & \mathbf{1}
    \end{pmatrix},~\text{and}~
    \mathbf{U} = \begin{pmatrix}
    \mathbf{0} & \mathbf{1} \\
    \mathbf{1} & \mathbf{0},
    \end{pmatrix}
\end{equation}
where $\mathbf{1} \in \{1\}^{2N \times 2N}$ and $\mathbf{0} \in \{0\}^{2N \times 2N}$.

\color{blue}
\begin{align*}
    a &= 3 (N - 2) (N - 3) p^4 + 
    2N (4N - 6) p (1 - p)^2 +
    N (N - 1) (1 - p)^4 \\    
    b &= (N - 2) (N - 3) p^3 ((N - 4) p - 1) + 
    N (3N - 5) p (1 - p)^2 (2 (N - 2) p - 1)
    \\&~~~~+
    N (N - 1) (N - 2) (1 - p)^4 \\
    &= 
    N^3 (1 - 4 p + 12 p^2 - 16 p^3 + 8 p^4) + 
    N^2 (-3 + 9 p - 34 p^2 + 52 p^3 - 34 p^4) 
    \\&~~~~+
    N (2 - 3 p + 22 p^2 - 38 p^3 + 48 p^4)
    -6 p^3 (1 + 4 p)
    \\
    c &= (N - 1) p^2 (1 - p) (4 (N - 2)^2 p - 3N + 5) + 
    (N - 1) (1 - p)^3 (4 (N - 2)^2 p - N + 1)
\end{align*}
Note: Here $p$ is from the training graphs.

% For $b$, for any $0.5 < p \leq 1$,
% \begin{align*}
%     1 - 4 p + 12 p^2 - 16 p^3 + 8 p^4 &> 0.5 \\
%     -3 + 9 p - 34 p^2 + 52 p^3 - 34 p^4 &\geq -10\\
%     2 - 3 p + 22 p^2 - 38 p^3 + 48 p^4 &> 4.25 \\
%     -6 p^3 (1 + 4 p) &\geq -30
% \end{align*}
% For any $N \geq 20$, 
% \[
% 0.5N^3 - 10N^2 + 4.25N - 30 > 0.
% \]

For any training graphs with $0.5 < p \leq 1$,
\begin{itemize}
    \item For any $N \geq 4$, $a > 0$
    \item For any $N \geq 6$, $b > 0$
    \item For any $N \geq 4$, $c > 0$,
\end{itemize}
so $a, b, c > 0$ for any $N \geq 6$.

\color{black}

Second, As shown in the above proof, for $p>0.5$ and $N \geq 4$, $\mathbb{E}_{A}[\mathbf{A}^{4} - \mathbf{A}^{3}]_{ij} > 0, \forall i,j \in [2N]$ holds. 
Thus, $a,b,c > 0$ holds.
Third, as mentioned in the statement of the theorem, we consider a very small learning rate $\gamma \approx 0$. 
Consequently, for the updated weight matrix $W'$, which is defined as $W' \coloneqq \mathbf{I} - \gamma \mathbb{E}_{A}[\mathbf{A}^{4} - \mathbf{A}^{3}]$, the following hold:
\begin{equation}
    W' = \mathbf{I} - \gamma (a\mathbf{I} + b\mathbf{P} + c\mathbf{U}) \coloneqq \mathbf{I} + \epsilon_{1}\mathbf{I} + \epsilon_{2}\mathbf{P} + \epsilon_{3}\mathbf{U}.
\end{equation}
where $\epsilon_{1} \coloneqq -\gamma a \lesssim 0 $, 
$\epsilon_{2} \coloneqq -\gamma b \lesssim 0 $, and 
$\epsilon_{3} \coloneqq -\gamma c \lesssim 0 $.
Note that $\epsilon_{1},\epsilon_{2}$, and $\epsilon_{3}$ are some small negative constants that are very close to zero.

Now, we derive the reconstruction loss that is computed with $W'$.
Formally, reconstruction loss by using $W'$ is defined as follows:
\begin{equation}\label{eq:theoryloss}
    \mathcal{L} = \lVert \mathbf{A} - \mathbf{A}W'(\mathbf{A}W')^{T}\rVert^{2}_{2} 
    = \lVert \mathbf{A} - \mathbf{A}(W')^{2}\mathbf{A}\rVert^{2}_{2}.
\end{equation}
Here, we further derive $(W')^{2}$ as follows:
\begin{equation}\label{eq:updatedgradientsquare}
    (W')^{2} = \mathbf{I} + 2(\epsilon_{1}\mathbf{I} + \epsilon_{2}\mathbf{P} + \epsilon_{3}\mathbf{U}) + (\epsilon_{1}\mathbf{I} + \epsilon_{2}\mathbf{P} + \epsilon_{3}\mathbf{U})^{2}.
\end{equation}
To simplify Eq.~(\ref{eq:updatedgradientsquare}), we use the property that $\mathbf{P}^{2} = N\mathbf{P}$, $\mathbf{U}^{2} = N\mathbf{U}$, and $\mathbf{PU}=\mathbf{UP} = N\mathbf{U}$.
We rewrite Eq.~(\ref{eq:updatedgradientsquare}) as below:
\begin{equation}\label{eq:simplifiedweight}
    (W')^{2} = \mathbf{I} + 2(\epsilon_{1}\mathbf{I} + \epsilon_{2}\mathbf{P} + \epsilon_{3}\mathbf{U}) + (\epsilon^{2}_{1}\mathbf{I} + \epsilon^{2}_{2}N\mathbf{P} + \epsilon^{2}_{3}N\mathbf{U}) + 2\epsilon_{1}\epsilon_{2}\mathbf{P} + 2\epsilon_{1}\epsilon_{3}\mathbf{U} + 2\epsilon_{2}\epsilon_{3}N\mathbf{U}.
\end{equation}
In Eq~(\ref{eq:simplifiedweight}), it is important to note that $\epsilon_{1},\epsilon_{2},\epsilon_{3} \approx \gamma$ and $\epsilon_{1}\epsilon_{2},\epsilon_{1}\epsilon_{3},\epsilon_{2}\epsilon_{3} \approx \gamma^{2}$.
This indicates that the coefficients of $\mathbf{I}$, $\mathbf{P}$, and $\mathbf{U}$ are governed by $1 + 2\epsilon_{1}$, $2\epsilon_{2}$, and $2\epsilon_{3}$, respectively.
Thus, we rewrite Eq~(\ref{eq:simplifiedweight}) as follows:
\begin{equation}
    (W')^{2} \equiv \mathbf{I} + \alpha_{1} \mathbf{I} + \alpha_{2} \mathbf{P}  + \alpha_{3} \mathbf{P},
\end{equation}
where $\alpha_{1}, \alpha_{2}, \alpha_{3} \lesssim 0$.

\color{blue}
\begin{align*}
    \alpha_1 &= 2 \epsilon_1 + \epsilon^2_1 \\
    \alpha_2 &= 2 \epsilon_2 + N\epsilon^2_2 + 2\epsilon_1 \epsilon_2 \\
    \alpha_3 &= 2 \epsilon_3 + N\epsilon^2_3 + 2\epsilon_1 \epsilon_3 + 2N \epsilon_2 \epsilon_3
\end{align*}
\color{black}

Now, by using the derived results, we rewrite the reconstruction loss term Eq~(\ref{eq:theoryloss}) as below:
\begin{equation}
    \mathcal{L} = \lVert \mathbf{A} - \mathbf{A}(\mathbf{I} + \alpha_{1} \mathbf{I} + \alpha_{2} \mathbf{P}  + \alpha_{3} \mathbf{P})\mathbf{A} \rVert^{2}_{F}
    = \lVert (\mathbf{A} - \mathbf{A}^{2}) - (\alpha_{1}\mathbf{A}^{2} + \alpha_{2}\mathbf{APA} + \alpha_{3}\mathbf{AUA})  \rVert^{2}_{F}.
\end{equation}

\color{blue}
\begin{align*}
    (\mathbf{APA})_{ij} &= \sum_{\text{$k, \ell$ in the same group}} \mathbf{A}_{ik} \mathbf{A}_{jl} \\
    (\mathbf{AUA})_{ij} &= \sum_{\text{$k, \ell$ in different groups}} \mathbf{A}_{ik} \mathbf{A}_{jl} \\
    (\mathbf{A}^2)_{ij} &= \sum_k \mathbf{A}_{ik} \mathbf{A}_{jk}
\end{align*}

\noindent\rule[0.5ex]{\linewidth}{1pt}

\[\mathcal{L} = \sum_{i, j} \mathcal{L}_{ij},\]
where
\[
\mathcal{L}_{ij} = \mathbf{A}_{ij} - (1 + \alpha_1)(\mathbf{A}^2)_{ij}
    - \alpha_2 (\mathbf{APA})_{ij}
    - \alpha_3 (\mathbf{AUA})_{ij}
    )^2.
\]
Let $x = A_{ij}$, $y = (\mathbf{A}^2)_{ij}$, $z = (\mathbf{APA})_{ij}$, and $w = (\mathbf{AUA})_{ij}$,
we have
\begin{align*}
    \mathcal{L}_{ij} 
    &= (
    x - (1 + \alpha_1)y
    - \alpha_2 z
    - \alpha_3 w
    )^2 \\
    &= x^2 + 
    - 2 (1 + \alpha_1) x y     
    - 2 \alpha_2 x z 
    - 2 \alpha_3 x w
    + (1 + \alpha_1)^2 y^2
    \\&~~~~+
    2 (1 + \alpha_1) \alpha_2 y z     
    + 2 (1 + \alpha_1) \alpha_3 y w    
    + \alpha_2^2 z^2
    + 2 \alpha_2 \alpha_3 z w
    + \alpha_3^2 w^2.
\end{align*}

Let 
\begin{align*}
    \bar{\mathcal{L}}_{ij} 
    &= (\mathbf{A}_{ij} - (\mathbf{A}^2)_{ij})^2 \\
    &= (x - y)^2,  
\end{align*}
we have
\begin{align*}
    \mathcal{L}_{ij} - \bar{\mathcal{L}}_{ij} 
    &= - 2 \alpha_1 x y
    - 2 \alpha_2 x z 
    - 2 \alpha_3 x w
    + \alpha_1 (\alpha_1 + 2) y^2
    \\&~~~~+
    2 (1 + \alpha_1) \alpha_2 y z     
    + 2 (1 + \alpha_1) \alpha_3 y w    
    + \alpha_2^2 z^2
    + 2 \alpha_2 \alpha_3 z w
    + \alpha_3^2 w^2.
\end{align*}
We shall show that 
\[
\mathbb{E} [\sum_{i, j} (\mathcal{L}_{ij} - \bar{\mathcal{L}}_{ij})] < 0.
\]

As $\gamma \to 0^+$, ignoring higher-order terms, it suffices to show that
\[
a (\mathbb{E}[xy] - \mathbb{E}[y^2]) + b(\mathbb{E}[xz] - \mathbb{E}[yz]) + c(\mathbb{E}[xw] - \mathbb{E}[yw]) < 0
\]
Note: In the following derivation, $p$ is from test graphs.

% Let $D_{ij} = \mathbf{A}_{ij} - (\mathbf{A}^2)_{ij} 
%     - \alpha_1 (\mathbf{A}^2)_{ij} 
%     - \alpha_2 (\mathbf{APA})_{ij}
%     - \alpha_3 (\mathbf{AUA})_{ij}$ (so that $\mathcal{L}_{ij} = D^2_{ij}$), we have
% \begin{equation*}
%     \mathbb{E} [\mathcal{L}_{ij}] 
%     = \mathbb{E} [{D}^2_{ij}]
%     = (\mathbb{E} [{D}_{ij}])^2 + \mathrm{Var}({D}_{ij}).
% \end{equation*}

\newpage

\subsubsection{(1) If $i = j$}

\begin{align*}
    x &\equiv 0\\
    \mathbb{E}[y] &= (N-1)p^2 + N(1-p)^2 = N (1 - 2p + 2p^2) - p^2 \\
    \mathbb{E}[z] &= (N-1)^2 p^2 + N^2(1-p)^2 = N^2 (1 - 2p + 2p^2) - 2 N p^2 + p^2 \\
    \mathbb{E}[w] &= 2 N (N-1) p (1-p) = 2 N^2 (p - p^2) + 2 N (p^2 - p)\\
    % \mathbb{E}[x^2] &= 0\\
    \mathbb{E}[xy] &= 0\\
    \mathbb{E}[xz] &= 0\\
    \mathbb{E}[xw] &= 0\\
    \mathbb{E}[y^2] &= 
    % \sum_{k, k'} A_{ik} A_{ik'}
    (N - 1) p  % k = k', S
    + (N - 1) (N - 2) p^2 % k \neq k', SS
    + N (1 - p) % k = k', D
    + N (N - 1) (1 - p)^2 % k \neq k', DD
    + 2 N (N - 1) p (1 - p) % k \neq k', DS/SD
    \\
    &= N^2 +
    N (-2p^2) +
    (2p^2 - p)    
    \\
    \mathbb{E}[yz] &= 
    % \sum_{k, t, l; t, l in the same group} A_{ik} A_{it} A_{il}
    (N - 1) (N - 2) (N - 3) p^3 + % S; SS; k, t, l all distinct
    3 (N - 1) (N - 2) p^2 + % S; SS; k \neq t = l or k = t \neq l or k = l \neq t    
    (N - 1) p % S; SS; k = t = l
    \\&~~~~+
    %
    N (N - 1)^2 p (1-p)^2 + % S; DD; t \neq l
    N (N - 1) p (1-p) % S; DD; t = l
    \\&~~~~+
    %
    N (N - 1) (N - 2) p^2 (1-p) + % D; SS; t \neq l
    N (N - 1) p (1 - p) % D; SS; t = l
    \\&~~~~+
    %
    N (N - 1) (N - 2) (1-p)^3 + % D; DD; k, t, l all distinct
    3 N (N - 1) (1-p)^2 + % D; DD; k \neq t = l or k = t \neq l or k = l \neq t    
    N (1 - p) % D; DD; k = t = l
    \\
    &= 
    N^3 (1 - 2 p + 2 p^2) + 
    N^2 (3p - 4 p^2 - 2 p^3)
    \\&~~~~+
    N (-p - 4 p^2 + 8 p^3) +
    (-p + 6 p^2 - 6 p^3)
    \\
    \mathbb{E}[yw] &= 
    % \sum_{k, t, l; t, l in diff. groups} A_{ik} A_{it} A_{il}
    2 N (N - 1) (N - 2) p^2 (1-p) + % S; DS/SD; k, t, l all distinct
    2 N (N - 1) p (1-p) % S; DS/SD; k = t or l
    \\&~~~~+
    2 N (N - 1)^2 p (1-p)^2 + % D; DS/SD; k, t, l all distinct
    2 N (N - 1) p (1-p) % D; DS/SD; k = t or l
    \\
    &=
    N^3 (2p - 2p^2) + 
    N^2 (2p^3 - 2p^2) +
    N (4 p^2 -2p - 2p^3)
    % \\
    % \mathbb{E}[z^2] &= 
    % % \sum_{k, l, k', l': k and l in the same group; k' and l' in the same group} A_{ik} A_{ik'} A_{il} A_{il'}
    % (N - 1) (N - 2) (N - 3) (N - 4) p^4 + % SS; SS; all distinct (1111)
    % 6 (N - 1) (N - 2) (N - 3) p^3  % SS; SS; 112
    % \\&~~~~+
    % 7 (N - 1) (N - 2) p^2 +  % SS; SS; 22 or 13    
    % (N - 1) p % SS; SS; 4
    % \\&~~~~+
    % 2 N (N - 1)^2 (N - 2) p^2 (1-p)^2 +  % SS; DD (or DD; SS); all distinct
    % 2 N (N - 1)^2 p (1-p)^2   % SS; DD (or DD; SS); SS same
    % \\&~~~~+
    % 2 N (N - 1) (N - 2) p^2 (1-p) +  % SS; DD (or DD; SS); DD same
    % 2 N (N - 1) p (1-p)   % SS; DD (or DD; SS); both SS and DD same
    % \\&~~~~+
    % % DD; DD; all distinct
    % N (N - 1) (N - 2) (N - 3) (1-p)^4 + % DD; DD; all distinct (1111)
    % 6 N (N - 1) (N - 2) (1-p)^3  % DD; DD; 112
    % \\&~~~~+
    % 7 N (N - 1) (1-p)^2 +  % DD; DD; 22 or 13
    % N (1-p) % DD; DD; 4    
    % \\
    % &=
    % N^4 (1 - 4 p + 8 p^2 - 8 p^3 + 4 p^4) + 
    % N^3 (8 p - 28 p^2 + 40 p^3 - 24 p^4)
    % \\&~~~~+
    % N^2 (-6 p + 36 p^2 - 80 p^3 + 56 p^4) +
    % N (2 p - 30 p^2 + 84 p^3 - 60 p^4)
    % \\&~~~~+
    % (-p + 14 p^2 - 36 p^3 + 24 p^4)
    % \\
    % \mathbb{E}[zw] &= 
    % % \sum_{k, l, k', l': k and l in the same group; k' and l' in diff groups} A_{ik} A_{ik'} A_{il} A_{il'}
    % 2 N (N - 1) (N - 2) (N - 3) p^3 (1 - p) + % SS; SD/DS; SSS 111
    % 6 N (N - 1) (N - 2) p^2 (1 - p) + % SS; SD/DS; SSS 12
    % 2 N (N - 1) p (1 - p) % SS; SD/DS; SSS 3
    % \\&~~~~+
    % 2 N (N - 1) (N - 2) (N - 1) p (1 - p)^3 + % DD; SD/DS; DDD 111
    % 6 N (N - 1) (N - 1) p (1 - p)^2 + % DD; SD/DS; DDD 12
    % 2 N (N - 1) p (1 - p) % DD; SD/DS; DDD 12
    % \\
    % &=
    % N^4 (2 p - 6 p^2 + 8 p^3 - 4 p^4) +
    % N^3 (-2 p + 18 p^2 - 36 p^3 + 20 p^4) 
    % \\&~~~~+
    % N^2 (2 p - 28 p^2 + 58 p^3 - 32 p^4) +
    % N (-2 p + 16 p^2 - 30 p^3 + 16 p^4)        
    % \\
    % \mathbb{E}[w^2] &=
    % % \sum_{k, l, k', l': k and l in diff. groups; k' and l' in diff groups} A_{ik} A_{ik'} A_{il} A_{il'}
    % 4N (N - 1) (N - 1) (N - 2) p^2 (1-p)^2 + % all distinct
    % 4N (N - 1) (N - 1) p (1-p)^2 % SS same
    % \\&~~~~+
    % 4N (N - 1) (N - 2) p^2 (1-p) + % DD same
    % 4N (N - 1) p (1-p) % both SS and DD same
    % \\
    % &=
    % N^4 (4 p^2 - 8 p^3 + 4 p^4) +
    % N^3 (4 p - 20 p^2 + 32 p^3 - 16 p^4) 
    % \\&~~~~+
    % N^2 (-4 p + 20 p^2 - 36 p^3 + 20 p^4) +
    % N (4p^3 - 4p^2) +
    % (4p^3 - 4p^2)
\end{align*}

Hence,
\begin{align*}
    d_{11} := \mathbb{E}[xy] - \mathbb{E}[y^2] &= -N^2 + N(2p^2) + (p-2p^2) \\
    d_{12} := \mathbb{E}[xz] - \mathbb{E}[yz] &= N^3 (-1 + 2 p - 2 p^2) + 
    N^2 (-3p + 4 p^2 + 2 p^3)
    \\&~~~~+
    N (p + 4 p^2 - 8 p^3) +
    (p - 6 p^2 + 6 p^3) \\
    d_{13} :=\mathbb{E}[xw] - \mathbb{E}[yw] &= 
    N^3 (-2p + 2p^2) + 
    N^2 (-2p^3 + 2p^2) +
    N (-4 p^2 +2p + 2p^3)
\end{align*}

% \begin{align*}
%     \mathbb{E}[xy] - \mathbb{E}[y^2] 
%     &= -N^2 + N(2p^2) + (p-2p^2) \\
%     &\leq -N^2 + 2N < 0, 
% \end{align*}
% for any $N \geq 3$;
% \begin{align*}
%     \mathbb{E}[xz] - \mathbb{E}[yz] &=
%     N^3 (-1 + 2 p - 2 p^2) + 
%     N^2 (-3p + 4 p^2 + 2 p^3)
%     \\&~~~~+
%     N (p + 4 p^2 - 8 p^3) +
%     (p - 6 p^2 + 6 p^3) \\
%     &\leq -0.5 N^3 + 3N^2 + 0.5N + 1 < 0,
% \end{align*}
% for any $N \geq 7$;
% \begin{align*}
%     \mathbb{E}[xw] - \mathbb{E}[yw] &= 
%     N^3 (-2p + 2p^2) + 
%     N^2 (-2p^3 + 2p^2) +
%     N (-4 p^2 +2p + 2p^3) \\
%     &\leq 
% \end{align*}

% Recall that we aim to show that 
% \[
% a (\mathbb{E}[xy] - \mathbb{E}[y^2]) + b(\mathbb{E}[xz] - \mathbb{E}[yz]) + c(\mathbb{E}[xw] - \mathbb{E}[yw]) < 0,
% \]
% where $a, b, c > 0$ for any $0.5 < p \leq 1$ and $N \geq 20$.



% Hence,
% \begin{align*}
%     \mathbb{E}[\mathcal{L}_{ij} - \bar{\mathcal{L}}_{ij}] 
%     &=
%     \mathbb{E}[x^2 + 
%     - 2 \alpha_1 x y
%     - 2 \alpha_2 x z 
%     - 2 \alpha_3 x w
%     + \alpha_1 (\alpha_1 + 2) y^2
%     \\&~~~~+
%     2 (1 + \alpha_1) \alpha_2 y z     
%     + 2 (1 + \alpha_1) \alpha_3 y w    
%     + \alpha_2^2 z^2
%     + 2 \alpha_2 \alpha_3 z w
%     + \alpha_3^2 w^2]  \\
%     &= \beta_{14} N^4 + \beta_{13} N^3 + \beta_{12} N^2 + \beta_{11} N^1 + \beta_{10} N^0,
% \end{align*}
% where
% \begin{equation*}
%     \beta_{14} = \alpha^2_2 (1 - 4 p + 8 p^2 - 8 p^3 + 4 p^4) + 2 \alpha_2 \alpha_3 (2 p - 6 p^2 + 8 p^3 - 4 p^4) + \alpha^2_3 (4 p^2 - 8 p^3 + 4 p^4)    
% \end{equation*}

% When $0.5 < p \leq 1$,
% \begin{align*}
%     0.25 < 1 - 4 p + 8 p^2 - 8 p^3 + 4 p^4 \leq 1 \\
%     0 \leq 2 p - 6 p^2 + 8 p^3 - 4 p^4 \leq 0.25 \\
%     0 \leq 4 p^2 - 8 p^3 + 4 p^4 \leq 0.25,
% \end{align*}
% so the highest coefficient
% \[
% \beta_{14} > 0.25 \alpha^2_2 > 0.
% \]

\newpage

\subsubsection{(2) Else if $i$ and $j$ are in the same group}

\begin{align*}
    \mathbb{E}[x] &= p \\
    \mathbb{E}[y] &= (N-2)p^2 + N(1-p)^2 = N (1 - 2p + 2p^2) - 2 p^2 \\    
    \mathbb{E}[z] &= (N-1)^2 p^2 + N^2(1-p)^2 = N^2 (1 - 2p + 2p^2) - 2 N p^2 + p^2 \\
    \mathbb{E}[w] &= 2 N (N-2) p (1-p) = 2 N^2 (p - p^2) + 4 N (p^2 - p) \\
    % \mathbb{E}[x^2] &= p\\
    \mathbb{E}[xy] &= p \mathbb{E}[y] = N p (1 - 2p + 2p^2) - 2 p^3 \\
    \mathbb{E}[xz] &= p \mathbb{E}[z] = N^2 p (1 - 2p + 2p^2) - 2 N p^3 + p^3 \\
    \mathbb{E}[xw] &= p \mathbb{E}[w] = 2 N^2 (p^2 - p^3) + 4 N (p^3 - p^2) \\
    \mathbb{E}[y^2] &=  
    % \sum_{k, k'} A_{ik} A_{ik'} A_{jk} A_{jk'}
    (N - 2) p^2 % k = k', S
    + (N - 2) (N - 3) p^4 % k \neq k', SS
    + N (1 - p)^2 % k = k', D
    + N (N - 1) (1 - p)^4 % k \neq k', DD
    + 2 N (N - 2) p^2 (1 - p)^2 % k \neq k', DS/SD
    \\
    &=
    N^2 (1 - 2 p + 2 p^2)^2 +
    2 N p (1 - 4 p + 6 p^2 - 5 p^3) +
    6 p^4 -2 p^2
    \\
    \mathbb{E}[yz] &=     
    % \sum_{k, t, l; t, l in the same group} A_{ik} A_{jk} A_{it} A_{jl}
    (N - 2) (N - 3) (N - 4) p^4 + % S; SS; k, t, l all distinct
    2 (N - 2) (N - 3) p^4 +       % S; SS; k, t, l all distinct; t = j or l = i    
    (N - 2) p^3                   % S; SS; k, t, l all distinct; t = j and l = i
    \\&~~~~+
    (N - 2) (N - 3) p^4 +         % S; SS; k \neq t = l
    2 (N - 2) (N - 3) p^3 +       % S; SS; k = t \neq l or k = l \neq t
    (N - 2) p^2                   % S; SS; k = t = l
    \\&~~~~+
    %
    N (N - 1) (N - 2) p^2 (1-p)^2 +     % S; DD; t \neq l
    N (N - 2) p^2 (1-p)                 % S; DD; t = l 
    \\&~~~~+
    %
    N (N - 2) (N - 3) p^2 (1-p)^2 +   % D; SS; t \neq l
    N (N - 2) p (1-p)^2               % D; SS; t = l
    \\&~~~~+
    %    
    N (N - 1) (N - 2) (1-p)^4 +     % D; DD; k, t, l all distinct    
    N (N - 1) (1-p)^4 +             % D; DD; k \neq t = l
    2 N (N - 1) (1-p)^3 +           % D; DD; k = t \neq l or k = l \neq t
    N (1-p)^2                       % D; DD; k = t = l
    \\
    &= 
    N^3 (1 - 2 p + 2 p^2)^2 - 
    2 p^2 (1 - 5 p + 3 p^2) 
    \\&~~~~+
    N^2 p (3 - 15 p + 24 p^2 - 16 p^3) + 
    N p (-2 + 12 p - 27 p^2 + 20 p^3)
    \\
    \mathbb{E}[yw] &= 
    % \sum_{k, t, l; t, l in diff. groups} A_{ik} A_{jk} A_{it} A_{jl}    
    2 N (N - 2) (N - 3) p^3 (1-p) + % S; DS/SD; k, t, l all distinct
    2 N (N - 2) p^3 (1-p) + % S; DS/SD; k, t, l all distinct; t = j or l = i    
    2 N (N - 2) p^2 (1-p)   % S; DS/SD; k = t or l
    \\&~~~~+
    2 N (N - 1) (N - 2) p (1-p)^3 + % D; DS/SD; k, t, l all distinct
    2 N (N - 2) p (1-p)^3 + % D; DS/SD; k, t, l all distinct; l = j or t = i
    2 N (N - 2) p (1-p)^2 % D; DS/SD; k = t or l
    \\
    &=
    N^3 (2 p - 6 p^2 + 8 p^3 - 4 p^4) +
    N^2 (-2 p + 10 p^2 - 20 p^3 + 12 p^4) +
    N (-4 p + 4 p^2 + 8 p^3 - 8 p^4)
\end{align*}


Hence,
\begin{align*}
    d_{21} := \mathbb{E}[xy] - \mathbb{E}[y^2] &= 
    -N^2 (1 - 2 p + 2 p^2)^2 +
    N p (-1 + 6 p - 10 p^2 + 10 p^3) +
    2 p^2 (1 - p - 3 p^2)  \\
    d_{22} := \mathbb{E}[xz] - \mathbb{E}[yz] &= 
    -N^3 (1 - 2 p + 2 p^2)^2 + p^2 (2 - 9 p + 6 p^2) 
    \\&~~~~+
    N p (2 - 12 p + 25 p^2 - 20 p^3) + 
    N^2 p (-2 + 13 p - 22 p^2 + 16 p^3)
    \\
    d_{23} := \mathbb{E}[xw] - \mathbb{E}[yw] &= 2 N (-1 + p) p (N (-1 + 3 p - 6 p^2) + N^2 (1 - 2 p + 2 p^2) + 
   2 (-1 + p + 2 p^2))
\end{align*}

% \newpage
% \begin{align*}
%     \mathbb{E}[z^2] &= 
%     % \sum_{k, l, k', l': k and l in the same group; k' and l' in the same group} A_{ik} A_{ik'} A_{jl} A_{jl'}
%     (N - 2) (N - 3) (N - 4) (N - 5) p^4 + % SS; SS; all distinct (1111)
%     4 (N - 2) (N - 3) (N - 4) p^4 + % SS; SS; all distinct (1111); k = j or k' = j or l = i or l' = i; only one
%     4 (N - 2) (N - 3) p^3 % SS; SS; all distinct (1111); (k = j or k' = j) and (l = i or l' = i); two
%     \\&~~~~+
%     %
%     2 (N - 2) (N - 3) (N - 4) p^3 + % SS; SS; 112; k = k' or l = l'
%     6 (N - 2) (N - 3)  p^3 + % SS; SS; 112; k = k' or l = l'; one side = i or j (1 + 2)
%     4 (N - 2) p^2 % SS; SS; 112; k = k' or l = l'; two sides = i or j (1 * 2)
%     \\&~~~~+
%     %
%     4 (N - 2) (N - 3) (N - 4) p^4 + % SS; SS; 112; k = l or k = l' or k' = l or k' = l'; 
%     8 (N - 2) (N - 3) p^4 + % SS; SS; 112; k = l or k = l' or k' = l or k' = l'; one side (only the remaining distinct two) = i or j (1 + 1)
%     4 (N - 2) p^3 % SS; SS; 112; k = l or k = l' or k' = l or k' = l'; two sides = i or j (1 * 1)
%     \\&~~~~+
%     %
%     (N - 2) (N - 3) p^2 + % SS; SS; 22; k = k' and l = l'    
%     2 (N - 2) p^2 + % SS; SS; 22; k = k' and l = l'; one side = i or j (1 + 1)
%     (N - 2) p % SS; SS; 22; k = k' and l = l'; two sides = i or j (1 * 1)
%     \\&~~~~+
%     %        
%     2 (N - 2) (N - 3) p^4 + % SS; SS; 22; (k = l and k' = l') or (k = l' and k' = l)
%     %
%     4 (N - 2) (N - 3) p^3 +  % SS; SS; 13
%     4 (N - 2) p^3 +  % SS; SS; 13; one side = i or j (only the "1" is possible)
%     %    
%     (N - 1) p^2 % SS; SS; 4
%     \\&~~~~+
%     %
%     2 N (N - 1) (N - 2) (N - 3) p^2 (1-p)^2 +  % SS; DD (or DD; SS); all distinct
%     2 N (N - 1) (N - 2) p^2 (1-p)^2   % SS; DD (or DD; SS); SS same
%     \\&~~~~+
%     2 N (N - 2) (N - 3) p^2 (1-p)^2 +  % SS; DD (or DD; SS); DD same
%     2 N (N - 2) p^2 (1-p)^2   % SS; DD (or DD; SS); both SS and DD same
%     \\&~~~~+
%     N (N - 1) (N - 2) (N - 3) (1-p)^4 + % DD; DD; all distinct (1111)    
%     2 N (N - 1) (N - 2) (1-p)^3  % DD; DD; 112; k = k' or l = l'
%     \\&~~~~+    
%     4 N (N - 1) (N - 2) (1-p)^4 + % DD; DD; 112; k = l or k = l' or k' = l or k' = l';    
%     N (N - 1) (1-p)^2 % DD; DD; 22; k = k' and l = l'    
%     \\&~~~~+    
%     2 N (N - 1) (1-p)^4 + % DD; DD; 22; (k = l and k' = l') or (k = l' and k' = l)
%     4 N (N - 1) (1-p)^3 + % DD; DD; 13
%     N (1-p)^2 % DD; DD; 4
%     \\
%     &=
%     N^4 (1 - 4 p + 8 p^2 - 8 p^3 + 4 p^4) + 
%     N^3 (2 p - 14 p^2 + 24 p^3 - 16 p^4)
%     \\&~~~~+    
%     N^2 (10 p^2 - 22 p^3 + 18 p^4) +
%     N p (1 + 2 p - 10 p^2 + 4 p^3) +
%     p (-2 - 7 p + 20 p^2 - 12 p^3)
%     \\
%     \mathbb{E}[zw] &= 
%     % \sum_{k, l, k', l': k and l in the same group; k' and l' in diff groups} A_{ik} A_{ik'} A_{jl} A_{jl'}
%     2 N (N - 2) (N - 3) (N - 4) p^3 (1 - p) + % SS; SD/DS; SSS 111
%     6 N (N - 2) (N - 3) p^3 (1 - p) + % SS; SD/DS; SSS 111; (k, k'), l; one side = i or j (2 + 1)
%     4 N (N - 2) p^2 (1 - p)  % SS; SD/DS; SSS 111; (k, k'), l; two sides = i or j (2 * 1)
%     \\&~~~~+
%     2 N (N - 2) (N - 3) p^2 (1 - p) + % SS; SD/DS; SSS 12; k = k'
%     2 N (N - 2) p^2 (1 - p) % SS; SD/DS; SSS 12; k = k' = j
%     \\&~~~~+
%     2 N (N - 2) p^2 (1 - p) + % SS; SD/DS; SSS 12; k = k'; l = i
%     2 N p (1 - p) % SS; SD/DS; SSS 12; k = k' = j; l = i
%     \\&~~~~+
%     4 N (N - 2) (N - 3) p^3 (1 - p) + % SS; SD/DS; SSS 12; k = l or k' = l
%     4 N (N - 2) p^3 (1 - p)  % SS; SD/DS; SSS 12; k = l or k' = l; remaining k' or k = i
%     \\&~~~~+
%     2 N (N - 2) p (1 - p) % SS; SD/DS; SSS 3
%     \\&~~~~+
%     2 N (N - 1) (N - 2) (N - 2) p (1 - p)^3 + % DD; SD/DS; DDD 111
%     6 N (N - 1) (N - 2) p (1 - p)^2 + % DD; SD/DS; DDD 12
%     2 N (N - 2) p (1 - p) % DD; SD/DS; DDD 12
%     \\
%     &=
%     N^4 (2 p - 6 p^2 + 8 p^3 - 4 p^4) +
%     N^3 (-4 p + 20 p^2 - 34 p^3 + 18 p^4) 
%     \\&~~~~+
%     N^2 (2 p - 18 p^2 + 38 p^3 - 22 p^4) +
%     N (-2 p + 2 p^2 - 4 p^3 + 4 p^4)
%     \\
%     \mathbb{E}[w^2] &=  
%     % \sum_{k, l, k', l': k and l in diff. groups; k' and l' in diff groups} A_{ik} A_{ik'} A_{jl} A_{jl'}
%     4N (N - 1) (N - 2) (N - 3) p^2 (1-p)^2 + % all distinct
%     8N (N - 1) (N - 2) p^2 (1-p)^2 + % all distinct; one side S = i or j 
%     4N (N - 1) p (1-p)^2 % all distinct; both sides S = i or j
%     \\&~~~~+    
%     4N (N - 1) (N - 2) p^2 (1-p)^2 % SS same
%     \\&~~~~+
%     4N (N - 2) (N - 3) p^2 (1-p)^2 + % DD same
%     8N (N - 2) p^2 (1-p)^2 + % DD same; one side S = i or j 
%     4N p (1-p)^2 % DD same; two sides S = i or j 
%     \\&~~~~+    
%     4N (N - 2) p^2 (1-p)^2 % both SS and DD same
%     \\
%     &=
%     N^4 (4 p^2 - 8 p^3 + 4 p^4) +
%     N^3 (-8 p^2 + 16 p^3 - 8 p^4) +
%     N^2 (4 p - 8 p^2 + 4 p^3)
% \end{align*}

% Hence,
% \begin{align*}
%     \mathbb{E}[\mathcal{L}_{ij} - \bar{\mathcal{L}}_{ij}] 
%     &=
%     \mathbb{E}[x^2 + 
%     - 2 \alpha_1 x y
%     - 2 \alpha_2 x z 
%     - 2 \alpha_3 x w
%     + \alpha_1 (\alpha_1 + 2) y^2
%     \\&~~~~+
%     2 (1 + \alpha_1) \alpha_2 y z     
%     + 2 (1 + \alpha_1) \alpha_3 y w    
%     + \alpha_2^2 z^2
%     + 2 \alpha_2 \alpha_3 z w
%     + \alpha_3^2 w^2] \\
%     &= \beta_{24} N^4 + \beta_{23} N^3 + \beta_{22} N^2 + \beta_{21} N^1 + \beta_{20} N^0,
% \end{align*}
% where
% \begin{equation*}
%     \beta_{24} = \alpha^2_2 (1 - 4 p + 8 p^2 - 8 p^3 + 4 p^4) + 2 \alpha_2 \alpha_3 (2 p - 6 p^2 + 8 p^3 - 4 p^4) + \alpha^2_3 (4 p^2 - 8 p^3 + 4 p^4)    
% \end{equation*}

% When $0.5 < p \leq 1$,
% \begin{align*}
%     0.25 < 1 - 4 p + 8 p^2 - 8 p^3 + 4 p^4 \leq 1 \\
%     0 \leq 2 p - 6 p^2 + 8 p^3 - 4 p^4 \leq 0.25 \\
%     0 \leq 4 p^2 - 8 p^3 + 4 p^4 \leq 0.25.
% \end{align*}
% There are $N (N - 1)$ same-group $(i, j)$-pairs.

\newpage

\subsubsection{(3) Else if $i$ and $j$ are in different groups}

\begin{align*}
    \mathbb{E}[x] &= 1 - p \\
    \mathbb{E}[y] &= 2(N-1)p(1-p) \\    
    \mathbb{E}[z] &= 2 (N - 1)^2 p (1 - p)\\
    \mathbb{E}[w] &= (N - 1)^2 p^2 + N^2 (1 - p)^2 \\
    % \mathbb{E}[x^2] &= 1 - p\\
    \mathbb{E}[xy] &= (1 - p) \mathbb{E}[y] = 2(N-1)p(1-p)^2\\
    \mathbb{E}[xz] &= (1 - p) \mathbb{E}[z] = 2 (N - 1)^2 p (1 - p)^2 \\
    \mathbb{E}[xw] &= (1 - p) \mathbb{E}[w] = (N - 1)^2 p^2 (1-p) + N^2 (1 - p)^3 \\
    \mathbb{E}[y^2] &= 
    % \sum_{k, k'} A_{ik} A_{ik'} A_{jk} A_{jk'}
    % suppose i in group 1 and j in group 2
    2(N - 1) p (1 - p) + % k = k', 1/2
    2(N - 1) (N - 2) p^2 (1 - p)^2 + % k \neq k', 11/22    
    2(N - 1)^2 p^2 (1 - p)^2 % k \neq k', 12/21
    \\
    &= 2(N - 1) p (1 - p) + 2(N - 1) (2N - 3) p^2 (1 - p)^2
    \\
    \mathbb{E}[yz] &= 
    % \sum_{k, t, l; t, l in the same group} A_{ik} A_{jk} A_{it} A_{jl}
    % suppose i in group 1 and j in group 2
    2 (N - 1) (N - 2) (N - 3) p^2 (1-p)^2 +     % 1; 11 (or 2; 22); k, t, l all distinct
    2 (N - 1) (N - 2) p^2 (1-p)^2               % 1; 11 (or 2; 22); k, t, l all distinct; l = i (or t = j)
    \\&~~~~+
    2 (N - 1) (N - 2) p^2 (1-p)^2 +             % 1; 11 (or 2; 22); k \neq t = l
    2 (N - 1) (N - 2) p (1-p)^2                 % 1; 11 (or 2; 22); k = t \neq l
    \\&~~~~+
    2 (N - 1) (N - 2) p^2 (1-p) +               % 1; 11 (or 2; 22); k = l \neq t
    2 (N - 1) p (1-p)                           % 1; 11 (or 2; 22); k = t = l
    \\&~~~~+
    %
    2 (N - 1)^2 (N - 2) p^2 (1-p)^2 +     % 1; 22 (or 2; 11); t \neq l
    2 (N - 1)^2 p^2 (1-p)^2               % 1; 22 (or 2; 11); t = l
    \\
    &=
    N^3 (4p^2 - 8p^3 + 4p^4) +
    N^2 (2p - 16p^2 + 28p^3 - 14p^4)
    \\&~~~~+
    N (-4p + 20p^2 - 32p^3 + 16p^4) +       
    2 p - 8 p^2 + 12 p^3 - 6 p^4
    \\
    \mathbb{E}[yw] &= 
    % \sum_{k, t, l; t, l in diff. groups} A_{ik} A_{jk} A_{it} A_{jl}    
    % suppose i in group 1 and j in group 2
    2 (N - 1)^2 (N - 2) p^3 (1-p) + % 1; 12; k, t, l all distinct    
    2 (N - 1)^2 p^2 (1-p)           % 1; 12; k = t
    \\&~~~~+
    2 (N - 1)^2 (N - 2) p (1-p)^3 + % 1; 21; k, t, l all distinct
    2 (N - 1)^2 p (1-p)^3           % 1; 21; k, t, l all distinct; l = i
    \\&~~~~+
    (N - 1) (N - 2) p (1-p)^3 +   % 1; 21; k, t, l all distinct; t = j
    (N - 1) p (1-p)^2             % 1; 21; k, t, l all distinct; l = i and t = j
    \\&~~~~+
    (N - 1)^2 p (1-p)^2 +         % 1; 21; k = l
    (N - 1) p (1-p)^2             % 1; 21; k = l; t = j
    \\
    &=
    N^3 (2 p - 6 p^2 + 8 p^3 - 4 p^4) +
    N^2 (-4 p + 15 p^2 - 24 p^3 + 13 p^4) 
    \\&~~~~+
    N (3 p - 13 p^2 + 23 p^3 - 13 p^4) +
    (-p + 4 p^2 - 7 p^3 + 4 p^4)
\end{align*}

Hence,
\begin{align*}
    d_{31} := \mathbb{E}[xy] - \mathbb{E}[y^2] &= -2 (-1 + N) (2 + 2 N (-1 + p) - 3 p) (-1 + p) p^2
    \\
    d_{32} := \mathbb{E}[xz] - \mathbb{E}[yz] &= -2 (-1 + N)^2 (2 + 2 N (-1 + p) - 3 p) (-1 + p) p^2
    \\
    d_{33} := \mathbb{E}[xw] - \mathbb{E}[yw] &= (-1 + p) (p (-1 + 2 p - 4 p^2) + 2 N^3 p (1 - 2 p + 2 p^2) 
    \\&~~~~+
   N p (3 - 8 p + 13 p^2) - N^2 (1 + 2 p - 9 p^2 + 13 p^3))
\end{align*}

\newpage
\subsubsection{Conclusion}

Now, it suffices to show that, for any $0.5 < p \leq 1$,
\[
d_{1i} + (N - 1) d_{2i} + N d_{3i} \leq 0, \forall i \in \{1,2,3\},
\]
and at least for one $i$ value the inequality is strict.
% \begin{align*}
% N d_{11} + N(N - 1) d_{21} + N^2 d_{31} &< 0 \\
% \end{align*}
Indeed,
\begin{align*}
    d_{11} + (N - 1) d_{21} + N d_{31} &=
    -N^4 (1 - 2 p + 2 p^2)^2 
    + 2 N p (-1 + 6 p - 12 p^2 + 10 p^3) 
    \\&~~~~+
    N^2 (-1 + 4 p - 17 p^2 + 29 p^3 - 26 p^4) 
    + N^3 (1 - 6 p + 17 p^2 - 22 p^3 + 16 p^4)
    \\&~~~~+
    (p - 4 p^2 + 9 p^3 - 6 p^4) < 0
    % &\leq -0.25N^4 + 6N^3 - 1.25N^2 + 6N + 0.5 < 0,    
\end{align*}
for any $N \geq 4$;
\begin{align*}
    d_{12} + (N - 1) d_{22} + N d_{32} &=
    N^4 (-1 + 4 p - 12 p^2 + 16 p^3 - 8 p^4) +
    N^3 p (-4 + 31 p - 56 p^2 + 34 p^3) 
    \\&~~~~+
    N^2 (p - 33 p^2 + 77 p^3 - 52 p^4) + 
    N p (-1 + 22 p - 52 p^2 + 32 p^3) 
    \\&~~~~+
    p - 8 p^2 + 15 p^3 - 6 p^4 < 0
    % \\    &\leq -0.5 N^4 + 5N^3 - 1.375 N^2 + N + 2 < 0,
\end{align*}
for any $N \geq 3$;
\begin{align*}
    d_{13} + (N - 1) d_{23} + N d_{33} &=
    N (-1 + p) (p - 12 p^3 + 4 N^3 p (1 - 2 p + 2 p^2) 
    \\&~~~~+
   N p (1 - 12 p + 33 p^2) - N^2 (1 + 4 p - 19 p^2 + 29 p^3)) < 0,
\end{align*}
for any $N \geq 2$.

% where $N > 0$, $-1 + p \leq 0$, and the remaining term
% \begin{align*}
%     4 N^3 p (1 - 2 p + 2 p^2) + 
%     N^2 (-1 - 4 p + 19 p^2 - 29 p^3) +
%     N p (1 - 12 p + 33 p^2) +
%     p - 12 p^3 
%     &\geq N^3 - 15 N^2 + 1.625 N - 11 \\
%     &> 0,
% \end{align*}
% for any $N \geq 15$.

In conclusion, when trained with any $0.5 < p_{train} \leq 1$ and $N_{train} \geq 6$ and
and tested with any $0.5 < p_{test} \leq 1$ and $N_{test} \geq 4$,
\begin{align*}
    d_1 := d_{11} + (N - 1) d_{21} + N d_{31} &< 0 \\
    d_2 := d_{12} + (N - 1) d_{22} + N d_{32} &< 0 \\
    d_3 := d_{13} + (N - 1) d_{23} + N d_{33} &\leq 0,
\end{align*}
and thus
% \[
% \frac{\partial \sum_{i, j} \mathbb{E}[\mathcal{L}_{ij} - \Bar{\mathcal{L}}_{ij}]}{\partial \gamma} < 0,
% \]
% equivalently,
\[
\lim_{\gamma \to 0^+} \sum_{i, j} \mathbb{E}[\mathcal{L}_{ij} - \Bar{\mathcal{L}}_{ij}] < 0,
\]
completing the proof.

\newpage

\subsection{Gradient speed}

\textbf{Settings:}
Training on graphs with $N$ and $0.5 < p' \leq 1$ and 
tested on graphs with $N$ and different $p$ values with $0.5 < p \leq 1$.

\textbf{Statement:}
For any $0.5 < p_1 \leq 0.99$ and $N \geq 17$,
if trained with $N$ and $p_1$,
then for any $p_2 \geq p_1 + 0.01$,
decrease with $p_2$ (i.e., $\mathbb{E} [\sum_{i, j} (\mathcal{L}_{ij} - \bar{\mathcal{L}}_{ij})]$) is larger than that with $p_1$.
% $\mathbb{E} [\sum_{i, j} (\mathcal{L}_{ij} - \bar{\mathcal{L}}_{ij})]$ decreases as $p$ increases, i.e., with larger $p$, reconstruction error decreases faster.
% Specifically, for any $0.5 < p' \leq 1$ and $N \geq 4$, the decrease with $0.5 < p_1 < p_2 \leq 1$ with $p_2 \geq p_1 + 0.01$, the decrease with $p_2$ is more than that with $p_1$.

\textbf{Proof:}
Regarding the ``speed'' of gradient,
\begin{align*}
    \frac{\partial d_1}{\partial p} &= 
    4 N^4 (1 - 4 p + 6 p^2 - 4 p^3) + 
    N^3 (-6 + 34 p - 66 p^2 + 64 p^3) 
    \\&~~~~+
    N^2 (4 - 34 p + 87 p^2 - 104 p^3) + 
    N (-2 + 24 p - 72 p^2 + 80 p^3) 
    \\&~~~~+
    (1 - 8 p + 27 p^2 - 24 p^3) \\
    \frac{\partial d_2}{\partial p} &=
    4 N^4 (1 - 2 p)^3 +  
    2 N^3 (-2 + 31 p - 84 p^2 + 68 p^3) 
    \\&~~~~+
    N^2 (1 - 66 p + 231 p^2 - 208 p^3) + 
    N (-1 + 44 p - 156 p^2 + 128 p^3) 
    \\&~~~~+
    (1 - 16 p + 45 p^2 - 24 p^3) \\
    \frac{\partial d_3}{\partial p} &=    
    4 N^4 (-1 + 2 p)^3 + 
    N^3 (3 - 46 p + 144 p^2 - 116 p^3) 
    \\&~~~~+
    N^2 (-1 + 26 p - 135 p^2 + 132 p^3) +
    N(-1 + 2 p + 36 p^2 - 48 p^3).
\end{align*}
% where $\frac{\partial d_1}{\partial p} < 0$ for any $N \geq 65$ and $0.51 \leq p \leq 1$.

\begin{align*}
    f(p, p', N) &:=\frac{\partial a d_1 + b d_2 + cd_2}{\partial p} \\
    &= a(N, p') \frac{\partial d_1(N, p)}{\partial p} + 
    b(N, p') \frac{\partial d_2(N, p)}{\partial p} + 
    c(N, p') \frac{\partial d_3(N, p)}{\partial p} \\
    &=
    -((-1 + N) N (-1 + 2 p + 36 p^2 - 48 p^3 + 4 N^3 (-1 + 2 p)^3 + 
      N^2 (3 - 46 p + 144 p^2 - 116 p^3) 
      \\&~~~~+
      N (-1 + 26 p - 135 p^2 + 132 p^3)) (-1 + p') (1 + 14 p' - 
      26 p'^2 + 32 p'^3 + 4 N^2 p' (1 - 2 p' + 2 p'^2) 
      \\&~~~~-
      N (1 + 14 p' - 28 p'^2 + 32 p'^3))) - (-1 + 8 p - 27 p^2 + 24 p^3 +
     N (2 - 24 p + 72 p^2 - 80 p^3) 
     \\&~~~~+
    N^3 (6 - 34 p + 66 p^2 - 64 p^3) + 
    4 N^4 (-1 + 4 p - 6 p^2 + 4 p^3) 
    \\&~~~~+
    N^2 (-4 + 34 p - 87 p^2 + 104 p^3)) (18 p'^4 + 
    N^2 (1 + 4 p' - 10 p'^2 + 4 p'^3 + 4 p'^4) 
    \\&~~~~-
    N (1 + 8 p' - 18 p'^2 + 8 p'^3 + 16 p'^4)) - (-1 + 16 p - 45 p^2 + 
    24 p^3 + 4 N^4 (-1 + 2 p)^3 
    \\&~~~~+
    N (1 - 44 p + 156 p^2 - 128 p^3) 
    \\&~~~~-
    2 N^3 (-2 + 31 p - 84 p^2 + 68 p^3) + 
    N^2 (-1 + 66 p - 231 p^2 + 208 p^3)) (-6 p'^3 (1 + 4 p') 
    \\&~~~~+
    N^2 (-3 + 9 p' - 34 p'^2 + 52 p'^3 - 34 p'^4) + 
    N^3 (1 - 4 p' + 12 p'^2 - 16 p'^3 + 8 p'^4) 
    \\&~~~~+
    N (2 - 3 p' + 22 p'^2 - 38 p'^3 + 48 p'^4)).
\end{align*}

Given $p_1$ and $p_2$,
% and $N \geq 17$,
% then for any $p_2 \geq p_1 + 0.01$,
\begin{align*}
    &~f(p_2, p_1, N) - f(p_1, p_1, N) \\
    &= 
    (-1 + N) N (-1 + p_1) (1 + 14 p_1 - 26 p_1^2 + 32 p_1^3 + 
    4 N^2 p_1 (1 - 2 p_1 + 2 p_1^2) 
    \\&~~~~-
    N (1 + 14 p_1 - 28 p_1^2 + 32 p_1^3)) (-1 + 2 p_1 + 36 p_1^2 - 
    48 p_1^3 + 4 N^3 (-1 + 2 p_1)^3 
    \\&~~~~+
    N^2 (3 - 46 p_1 + 144 p_1^2 - 116 p_1^3) + 
    N (-1 + 26 p_1 - 135 p_1^2 + 132 p_1^3)) 
    \\&~~~~+
    (-1 + 8 p_1 - 27 p_1^2 + 
    24 p_1^3 + N (2 - 24 p_1 + 72 p_1^2 - 80 p_1^3) + 
    N^3 (6 - 34 p_1 + 66 p_1^2 - 64 p_1^3) 
    \\&~~~~+
    4 N^4 (-1 + 4 p_1 - 6 p_1^2 + 4 p_1^3) 
    \\&~~~~+
    N^2 (-4 + 34 p_1 - 87 p_1^2 + 104 p_1^3)) (18 p_1^4 + 
    N^2 (1 + 4 p_1 - 10 p_1^2 + 4 p_1^3 + 4 p_1^4) 
    \\&~~~~-
    N (1 + 8 p_1 - 18 p_1^2 + 8 p_1^3 + 16 p_1^4)) + (-1 + 16 p_1 - 
    45 p_1^2 + 24 p_1^3 + 4 N^4 (-1 + 2 p_1)^3 
    \\&~~~~+
    N (1 - 44 p_1 + 156 p_1^2 - 128 p_1^3) - 
    2 N^3 (-2 + 31 p_1 - 84 p_1^2 + 68 p_1^3) 
    \\&~~~~+
    N^2 (-1 + 66 p_1 - 231 p_1^2 + 208 p_1^3)) (-6 p_1^3 (1 + 4 p_1) + 
    N^2 (-3 + 9 p_1 - 34 p_1^2 + 52 p_1^3 - 34 p_1^4) 
    \\&~~~~+
    N^3 (1 - 4 p_1 + 12 p_1^2 - 16 p_1^3 + 8 p_1^4) + 
    N (2 - 3 p_1 + 22 p_1^2 - 38 p_1^3 + 48 p_1^4)) 
    \\&~~~~-
    (18 p_1^4 + 
    N^2 (1 + 4 p_1 - 10 p_1^2 + 4 p_1^3 + 4 p_1^4) 
    \\&~~~~-
    N (1 + 8 p_1 - 18 p_1^2 + 8 p_1^3 + 16 p_1^4)) (-1 + 8 p_2 - 27 p_2^2 + 
    24 p_2^3 + N (2 - 24 p_2 + 72 p_2^2 - 80 p_2^3) 
    \\&~~~~+
    N^3 (6 - 34 p_2 + 66 p_2^2 - 64 p_2^3) + 
    4 N^4 (-1 + 4 p_2 - 6 p_2^2 + 4 p_2^3) 
    \\&~~~~+
    N^2 (-4 + 34 p_2 - 87 p_2^2 + 104 p_2^3)) - (-1 + N) N (-1 + 
    p_1) (1 + 14 p_1 - 26 p_1^2 + 32 p_1^3 
    \\&~~~~+
    4 N^2 p_1 (1 - 2 p_1 + 2 p_1^2) - 
    N (1 + 14 p_1 - 28 p_1^2 + 32 p_1^3)) (-1 + 2 p_2 + 36 p_2^2 
    \\&~~~~-
    48 p_2^3 + 4 N^3 (-1 + 2 p_2)^3 
    \\&~~~~+
    N^2 (3 - 46 p_2 + 144 p_2^2 - 116 p_2^3) + 
    N (-1 + 26 p_2 - 135 p_2^2 + 132 p_2^3)) - (-6 p_1^3 (1 + 4 p_1) 
    \\&~~~~+
    N^2 (-3 + 9 p_1 - 34 p_1^2 + 52 p_1^3 - 34 p_1^4) 
    \\&~~~~+
    N^3 (1 - 4 p_1 + 12 p_1^2 - 16 p_1^3 + 8 p_1^4) + 
    N (2 - 3 p_1 + 22 p_1^2 - 38 p_1^3 + 48 p_1^4)) (-1 + 16 p_2 
    \\&~~~~-
    45 p_2^2 + 24 p_2^3 + 4 N^4 (-1 + 2 p_2)^3 
    \\&~~~~+
    N (1 - 44 p_2 + 156 p_2^2 - 128 p_2^3) - 
    2 N^3 (-2 + 31 p_2 - 84 p_2^2 + 68 p_2^3) 
    \\&~~~~+
    N^2 (-1 + 66 p_2 - 231 p_2^2 + 208 p_2^3))
\end{align*}

By analyzing the above equation, we can find that 
when $N \geq 17$, $0.5 < p_1 \leq 0.99$, and $p_1 + 0.01 \leq p_2 \leq 1$,
the above equation is negative, i.e., $f(p_2, p_1, N) - f(p_1, p_1, N) < 0$, completing the proof.



% For the other two terms,
% \begin{align*}
%     b - c &=
%     N'^3 (1 - 2 p')^4 +
%     2 N'^2 (-1 + 13 p' - 44 p'^2 + 64 p'^3 - 37 p'^4) 
%     \\&~~~~+
%     N' p' (-29 + 104 p' - 156 p'^2 + 112 p'^3) + 
%     (1 + 13 p' - 40 p'^2 + 52 p'^3 - 56 p'^4) \\
%     &\geq 0.335 - 0.857 N' + 0.344 N'^2 + 1.6 \times 10^{-7} N'^3
%     % &\geq 3.159
% \end{align*}
% for all $N' \geq 35$ and $0.51 \leq p' \leq 1$,
% where $p'$ and $N'$ are from training graphs.
% Note that $b = \Omega(N'^3)$ and $c = \Omega(N'^3)$ have the same highest order.

% We thus have
% \begin{align*}
%     \frac{\partial a d_1 + b d_2 + cd_2}{\partial p}
%     &= a \frac{\partial d_1}{\partial p} + 
%     b \frac{\partial d_2}{\partial p} + 
%     c \frac{\partial d_3}{\partial p} \\
%     &< b \frac{\partial d_2}{\partial p} + 
%     c \frac{\partial d_3}{\partial p} \\
%     &< 4 (b-c) N^4 (1 - 2 p)^3 + \max(b, c) O(N^3),
% \end{align*}
% where $(b - c) (-1 + 2 p)^3 < 0$.
% Hence, for large enough $N$, the value of $4 (b-c) N^4 (1 - 2 p)^3 + \max(b, c) O(N^3)$ is dominated by $4 (b-c) N^4 (1 - 2 p)^3 < 0$, either when we fix $N'$ as a constant or use $N = N'$ (since $b = \Omega(N'^3)$, $c = \Omega(N'^3)$, and $b - c = \Omega(N'^3)$, the highest-order term still has coefficient $4 (b-c) (1 - 2 p)^3$).



% a; coef 3 = 
% b; coef 3 = (1 - 4 p + 12 p^2 - 16 p^3 + 8 p^4)
% c; coef 3 = 4p - 12p^2 + 16p^3 - 8p^4



% \newpage
% \begin{align*}
%     \mathbb{E}[z^2] &= 
%     % \sum_{k, l, k', l': k and l in the same group; k' and l' in the same group} A_{ik} A_{ik'} A_{jl} A_{jl'}
%     % suppose i in group 1 and j in group 2    
%     2 (N - 1) (N - 2) (N - 3) (N - 4) p^2 (1-p)^2 + % 11; 11; all distinct (1111)
%     4 (N - 1) (N - 2) (N - 3) p^2 (1-p)^2  % 11; 11; all distinct (1111); l = i or l' = i; only one    
%     \\&~~~~+
%     %
%     2 (N - 1) (N - 2) (N - 3) p (1-p)^2 + % 11; 11; 112; k = k'
%     4 (N - 1) (N - 2) p (1-p)^2  % 11; 11; 112; k = k'; l = i or l' = i
%     \\&~~~~+
%     2 (N - 1) (N - 2) (N - 3) p^2 (1-p) + % 11; 11; 112; l = l'
%     2 (N - 1) (N - 2) p^2 (1-p)  % 11; 11; 112; l = l' = i
%     \\&~~~~+
%     8 (N - 1) (N - 2) (N - 3) p^2 (1-p)^2 + % 11; 11; 112; k = l or k = l' or k' = l or k' = l'; 
%     8 (N - 1) (N - 2) p^2 (1 - p)^2  % 11; 11; 112; k = l or k = l' or k' = l or k' = l'; the other l = i    
%     \\&~~~~+    
%     2 (N - 1) (N - 2) p (1-p) + % 11; 11; 22; k = k' and l = l'
%     2 (N - 1) p (1-p) % 11; 11; 22; k = k' and l = l' = i
%     \\&~~~~+                
%     4 (N - 1) (N - 2) p^2 (1-p)^2 + % 11; 11; 22; (k = l and k' = l') or (k = l' and k' = l)
%     4 (N - 1) (N - 2) p^2 (1-p)   % 11; 11; 13; k or k' isolated    
%     \\&~~~~+                
%     4 (N - 1) (N - 2) p (1-p)^2 +  % 11; 11; 13; l or l' isolated
%     4 (N - 1) p (1-p)^2 +  % 11; 11; 13; l or l' isolated; isolated = i        
%     2 (N - 1) p (1-p) % 11; 11; 4
%     \\&~~~~+    
%     2 (N - 1)^2 (N - 2)^2 p^2 (1-p)^2 +  % 11; 22
%     4 (N - 1)^2 (N - 2) p^2 (1-p)^2 +     % 11; 22; 11 same or 22 same
%     2(N - 1)^2 p^2 (1-p)^2      % 11; 22; 11 same and 22 same    
%     \\
%     &=
%     N^4 (4p^2 - 8 p^3 + 4p^4) +
%     N^3 (2 p - 18 p^2 + 32 p^3 - 16 p^4) 
%     \\&~~~~+    
%     N^2 (-2 p + 22 p^2 - 42 p^3 + 22 p^4) +
%     N (-10 p^2 + 22 p^3 - 12 p^4) +        
%     (2 p^2 - 4 p^3 + 2 p^4)
%     \\
%     \mathbb{E}[zw] &= 
%     % \sum_{k, l, k', l': k and l in the same group; k' and l' in diff groups} A_{ik} A_{ik'} A_{jl} A_{jl'}
%     % suppose i in group 1 and j in group 2
%     2(N - 1) (N - 2) (N - 3) (N - 1) p^3 (1-p) +  % 11; 12; 111 (k k' l)
%     2(N - 1) (N - 2) (N - 1) p^3 (1-p)  % 11; 12; 111; l = i
%     \\&~~~~+
%     2(N - 1) (N - 2) (N - 1) p^2 (1-p) + % 11; 12; k = k' \neq l    
%     2(N - 1) (N - 1) p^2 (1-p) % 11; 12; k = k' \neq l; l = i    
%     \\&~~~~+
%     4 (N - 1) (N - 2) (N - 1) p^3 (1-p)  % 11; 12; k = l or k' = l; k \neq k'
%     \\&~~~~+
%     2(N - 1) (N - 1) p^2 (1-p) % 11; 12; k = k' = l
%     \\&~~~~+
%     2(N - 1) (N - 2) (N - 3) (N - 1) p (1-p)^3 + % 11; 21; 111 (k l l')
%     4 (N - 1) (N - 2) (N - 1) p (1-p)^3  % 11; 21; 111 (k l l'); l or l' = i
%     \\&~~~~+
%     2(N - 1) (N - 2) (N - 1) p (1-p)^2 + % 11; 21; l = l' \neq k
%     2(N - 1) (N - 1) p (1-p)^2  % 11; 21; l = l' \neq k; l = l' = i
%     \\&~~~~+
%     4 (N - 1) (N - 2) (N - 1) p (1-p)^3  % 11; 21; k = l or k = l'; l \neq l'
%     \\&~~~~+
%     2(N - 1) (N - 1) p (1-p)^2 % 11; 21; k = l = l'
%     \\
%     &= 
%     N^4 (2 p - 6 p^2 + 8 p^3 - 4 p^4) +
%     N^3 (-4 p + 16 p^2 - 26 p^3 + 14 p^4) 
%     \\&~~~~+
%     N^2 (-2 p - 2 p^2 + 16 p^3 - 12 p^4) +
%     N (8 p - 20 p^2 + 14 p^3 - 2 p^4) 
%     \\&~~~~+
%     (-4 p + 12 p^2 - 12 p^3 + 4 p^4)    
%     \\
%     \mathbb{E}[w^2] &=
%     % \sum_{k, l, k', l': k and l in diff. groups; k' and l' in diff groups} A_{ik} A_{ik'} A_{jl} A_{jl'}
%     % suppose i in group 1 and j in group 2
%     (N - 1) (N - 2) (N - 1) (N - 2) p^4 + % 12; 12; all distinct
%     2 (N - 1) (N - 1) (N - 2) p^3 + % 12; 12; 11 same or 22 same
%     (N - 1) (N - 1) p^2 % 12; 12; both 11 and 22 same
%     \\&~~~~+    
%     2 (N - 1) (N - 2) (N - 1) (N - 2) p^2 (1-p)^2 + % 12; 21 or 21; 12
%     4 (N - 1) (N - 1) (N - 2) p^2 (1-p)^2  % 12; 21 or 21; 12; one side = i or j 
%     \\&~~~~+
%     2 (N - 1) (N - 1) p^2 (1-p) + % 12; 21 or 21; 12; two sides = i or j
%     4 (N - 1) (N - 2) (N - 1) p^2 (1-p)^2 + % 12; 21 or 21; 12; 11 same or 22 same    
%     2 (N - 1) (N - 1) p^2 (1-p)^2  % 12; 21 or 21; 12; both 11 and 22 same
%     \\&~~~~+
%     % 21; 21
%     (N - 1) (N - 2) (N - 1) (N - 2) (1-p)^4 + % 21; 21; all distinct
%     2 (N - 1) (N - 1) (N - 2) (1-p)^3  % 21; 21; 11 same or 22 same
%     \\&~~~~+
%     2 (N - 1) (N - 2) (1-p)^3 + % 21; 21; 11 same or 22 same; same side = i or j
%     4 (N - 1) (N - 1) (1-p)^3 + % 21; 21; 11 same or 22 same; diff side = i or j
%     2 (N - 1) (1-p)^2  % 21; 21; 11 same or 22 same; both sides = i or j
%     \\&~~~~+    
%     (N - 1) (N - 1) (1-p)^2 + % 21; 21; both 11 and 22 same
%     2 (N - 1) (1-p)^2 + % 21; 21; both 11 and 22 same; one side = i or j 
%     (1-p) % 21; 21; both 11 and 22 same; two sides = i or j
%     \\
%     &=
%     N^4 (1 - 4 p + 8 p^2 - 8 p^3 + 4 p^4) +
%     N^3 (-4 + 18 p - 34 p^2 + 32 p^3 - 16 p^4) 
%     \\&~~~~+    
%     N^2 (12 - 48 p + 72 p^2 - 52 p^3 + 22 p^4) +
%     N (-14 + 56 p - 76 p^2 + 42 p^3 - 12 p^4) 
%     \\&~~~~+    
%     (6 - 23 p + 30 p^2 - 14 p^3 + 2 p^4 )    
% \end{align*}

% \newpage

% Hence,
% \begin{align*}
%     \mathbb{E}[\mathcal{L}_{ij} - \bar{\mathcal{L}}_{ij}] 
%     &=
%     \mathbb{E}[x^2 + 
%     - 2 \alpha_1 x y
%     - 2 \alpha_2 x z 
%     - 2 \alpha_3 x w
%     + \alpha_1 (\alpha_1 + 2) y^2
%     \\&~~~~+
%     2 (1 + \alpha_1) \alpha_2 y z     
%     + 2 (1 + \alpha_1) \alpha_3 y w    
%     + \alpha_2^2 z^2
%     + 2 \alpha_2 \alpha_3 z w
%     + \alpha_3^2 w^2] \\
%     &= \beta_{34} N^4 + \beta_{33} N^3 + \beta_{32} N^2 + \beta_{31} N^1 + \beta_{30} N^0,
% \end{align*}
% where
% \begin{equation*}
%     \beta_{34} = \alpha^2_2 (4p^2 - 8 p^3 + 4p^4) + 2 \alpha_2 \alpha_3 (2 p - 6 p^2 + 8 p^3 - 4 p^4) + \alpha^2_3 (1 - 4 p + 8 p^2 - 8 p^3 + 4 p^4)    
% \end{equation*}

% When $0.5 < p \leq 1$,
% \begin{align*}
%     0.25 < 1 - 4 p + 8 p^2 - 8 p^3 + 4 p^4 \leq 1 \\
%     0 \leq 2 p - 6 p^2 + 8 p^3 - 4 p^4 \leq 0.25 \\
%     0 \leq 4 p^2 - 8 p^3 + 4 p^4 \leq 0.25.
% \end{align*}
% There are $N (N - 1)$ same-group $(i, j)$-pairs.

\color{black}

% \red{In general, it is expected that each entry of $\mathbf{A} - \mathbf{A}^{2}$ is negative.
% On the other hand, each entry of $\alpha_{1}\mathbf{A}^{2} + \alpha_{2}\mathbf{APA} + \alpha_{3}\mathbf{AUA}$ is greater than zero, but very close to zero.
% Overall, it is expected that each entry of $((\mathbf{A} - \mathbf{A}^{2}) - (\alpha_{1}\mathbf{A}^{2} + \alpha_{2}\mathbf{APA} + \alpha_{3}\mathbf{AUA}))^{2}$ is smaller than $(\mathbf{A} - \mathbf{A}^{2})^{2}$.}


% \subsection{Global minimum}

% \textbf{Settings:}
% Trained on $p = 0.5$, i.e., Erdos-Renyi random graphs with $n = 2N$ and $p = 0.5$.
% Tested on $p = 1$, i.e., a block matrix.

% The loss is
% \[
% \mathcal{L} = \lVert \mathbf{A} - \mathbf{A} W W^T \mathbf{A}\rVert^{2}_{F} = \sum_{i, j} \mathcal{L}_{ij},
% \]
% % \begin{align*}
% %     \mathcal{L} 
% %     &= \lVert \mathbf{A} - \mathbf{A} W W^T \mathbf{A}\rVert^{2}_{F} 
% % \end{align*}
% where
% \[
% \mathcal{L}_{ij} = (\mathbf{A} - \mathbf{A} W W^T \mathbf{A})_{ij}^2.
% \]
% The expected value of each $\mathbb{E} \mathbf{A}_{ij} = \frac{1}{2}$, and we want to minimize each
% \[
% \mathcal{L}_{ij} = \mathbf{A}_{ij} - (\mathbf{A} W W^T \mathbf{A})_{ij} \left((\mathbf{A} W W^T \mathbf{A})_{ij} - 2 \mathbf{A}^_{ij}\right).
% \]
% Hence, we need to make
% \[
% (\mathbf{A} W W^T \mathbf{A})_{ij} = \mathbf{A}^_{ij}.
% \]
% By symmetry, we need $W_{ij} \equiv 2 n^{-3/2}$ so that
% \[
% (\mathbf{A} W W^T \mathbf{A})_{ij} \equiv \frac{1}{2}
% \]




